MetaGraphLoc: A Graph-based Meta-learning Scheme for Indoor Localization via Sensor Fusion

Accurate indoor localization remains challenging due to variations in wireless signal environments and limited data availability. This paper introduces MetaGraphLoc, a novel system leveraging sensor fusion, graph neural networks (GNNs), and meta-learning to overcome these limitations. MetaGraphLoc integrates received signal strength indicator measurements with inertial measurement unit data to enhance localization accuracy. Our proposed GNN architecture, featuring dynamic edge construction (DEC), captures the spatial relationships between access points and underlying data patterns. MetaGraphLoc employs a meta-learning framework to adapt the GNN model to new environments with minimal data collection, significantly reducing calibration efforts. Extensive evaluations demonstrate the effectiveness of MetaGraphLoc. Data fusion reduces localization error by 15.92%, underscoring its importance. The GNN with DEC outperforms traditional deep neural networks by up to 30.89%, considering accuracy. Furthermore, the meta-learning approach enables efficient adaptation to new environments, minimizing data collection requirements. These advancements position MetaGraphLoc as a promising solution for indoor localization, paving the way for improved navigation and location-based services in the ever-evolving Internet of Things networks.

==> common/biography.tex <==
\vspace{11pt}

\bf{If you include a photo:}\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
Use the author name as the 3rd argument followed by the biography text.
\end{IEEEbiography}

\vspace{11pt}

\bf{If you will not include a photo:}\vspace{-33pt}
\begin{IEEEbiographynophoto}{John Doe}
Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
\end{IEEEbiographynophoto}

\vfill

==> draft.tex <==
\section{Draft}


\subsection{Graph NN Loc}
Overall, GNNs offer a promising approach for enhancing the accuracy and robustness of fingerprinting-based indoor localization systems. Their ability to capture spatial relationships, incorporate structural information, and handle data heterogeneity make them well-suited for this domain.

\subsection{Factor Graph Neural Networks FaGCNLoc}
\textbf{1. Define the Variables:}

Let \( X_t \) be the set of unknown variables representing the location of the mobile device or target at time \( t \). For example, \( X_t = \{x_t, y_t, z_t\} \) for a three-dimensional location at time \( t \).

Let \( Z_t^{AP} \) be the set of observed variables representing the RSSI measurements from available Access Points at time \( t \). Each element \( Z_t^{AP_i} \) corresponds to the RSSI from the \( i \)-th Access Point at time \( t \).

Let \( Z_t^{IMU} \) be the set of observed variables representing IMU sensor readings at time \( t \). These could include acceleration, gyroscope, or other relevant measurements.

\textbf{2. Define the Factors:}

For the AP observations, let \( f_t^{AP_i}(X_t) \) be a factor representing the relationship between the location \( X_t \) and the RSSI measurement \( Z_t^{AP_i} \) from the \( i \)-th Access Point at time \( t \).

For the IMU observations, let \( f_t^{IMU}(X_t) \) be a factor representing the relationship between the location \( X_t \) and the IMU sensor readings \( Z_t^{IMU} \) at time \( t \).

\textbf{3. Construct the Factor Graph:}

The factor graph will have variable nodes corresponding to \( X_t \) and \( Z_t \) (both \( Z_t^{AP} \) and \( Z_t^{IMU} \)), and factor nodes corresponding to \( f_t^{AP_i} \) and \( f_t^{IMU} \).

Connect variable nodes to the corresponding factor nodes based on the relationships defined by the factors. For example, \( X_t \) would be connected to both \( f_t^{AP_i} \) and \( f_t^{IMU} \), and \( Z_t^{AP_i} \) would be connected to \( f_t^{AP_i} \).

\textbf{4. Define the Energy Function:}

The energy function \( E(X_t, Z_t) \) will be a sum of terms corresponding to each factor. For example:
\[
E(X_t, Z_t) = \sum_{i} E_t^{AP_i}(X_t, Z_t^{AP_i}) + E_t^{IMU}(X_t, Z_t^{IMU})
\]
where \( E_t^{AP_i} \) and \( E_t^{IMU} \) are the energy terms corresponding to the AP and IMU factors at time \( t \).

\textbf{5. Integrate Neural Networks:}

If you're using neural networks in your FGNN, you can incorporate them into the factor nodes \( f_t^{AP_i} \) and \( f_t^{IMU} \) to capture complex relationships and non-linearities. For example, the output of a neural network can be used as a factor in the energy function.

\textbf{6. Objective Function:}

The objective function is to minimize the energy function:
\[
\text{Minimize } E(X_t, Z_t)
\]

\textbf{7. Optimization:}

Use optimization algorithms such as gradient descent or other suitable methods to find the values of \( X_t \) that minimize the objective function.




==> progress.tex <==
\section{Graph-based RSSI Localization}
In this part the localization problem is formulated as a graph learning problem where the nodes represent the APs in the wireless environment.
IN this approach, the graph formulation allows features extraction taking into account the relationship between different APs, catching their spatial relationship and the part of the overall network geometry. 
Here the graph is represented by G(V,E), where V is the set of APs and E is the pairwise relations between APs.

Each RSSI measurement at a given timestamp is represented by the graph which is mapped to the corresponding reference position.

The overall model comprises the graph convolution layers for feature extraction followed by fully connected layers.

\section{System Model}
AP graphs. 
See Fig. \ref{fig:sysm}\\
\begin{itemize}
    \item AP cooperation for user localization
    \item Exploiting IoT network topology/geometry to assist user localization
    \item Region/context-aware localization
\end{itemize}
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.5]{temp_figures/system_model.png}
    \caption{Caption}
    \label{fig:sysm}
\end{figure}

\section{Data exploration}
See Fig. \ref{fig:dataviz}
\begin{figure*}[h]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\linewidth]{temp_figures/3D_scatter_plot_2024-01-24_20-35-01.png}
        \caption{Full trajectories}
        \label{fig:subfig1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\linewidth]{temp_figures/3D_scatter_plot_2024-01-24_20-37-12.png}
        \caption{Sampled trajectories}
        \label{fig:subfig2}
    \end{subfigure}
    \caption{Dataset visualization}
    \label{fig:dataviz}
\end{figure*}

\section{Graph architecture search}



